Graph Neural Reasoning for 2-Quantified Boolean Formula Solvers

In this paper, we investigate the feasibility of learning GNN (Graph Neural Network) based solvers and GNN-based heuristics for specified QBF (Quantified Boolean Formula) problems. We design and evaluate several GNN architectures for 2QBF formulae, and conjecture that GNN has limitations in learning 2QBF solvers. Then we show how to learn a heuristic CEGAR 2QBF solver. We further explore generalizing GNN-based heuristics to larger unseen instances, and uncover some interesting challenges. In summary, this paper provides a comprehensive surveying view of applying GNN-embeddings to specified QBF solvers, and aims to offer guidance in applying ML to more complicated symbolic reasoning problems.

==> supple_20_main.tex <==
% The obvious difference between SAT and 2QBF is that in 2QBF the literals are
% quantified by $\forall$ or $\exists$. We propose our GNN embedding
% architectures for 2QBF formulae, based on the known embedding of SAT
% \citep{DBLP:journals/corr/abs-1802-03685}, but uses
% different embedding matrices and NN modules for the $\forall$- and
% $\exists$-quantifed literals.

% The simplest form of embedding (Model 1) is given below. 
\section{All GNN-embedding Architectures}

We use subscript symbols
  $\forall$ to denote all $\forall$-quantified literals,
  $\exists$ to denote all $\exists$-quantified literals,
  $L$ to denote all literals, and $C$ to denote all clauses. 
  We use notations
$\text{Emb}_{X}$ to denote embeddings of $X$, where $X$ can be subscript
$\forall$, $\exists$, $L$, or $C$. We use notations
$\text{Emb}_{\neg X}$ to denote embedding of the negations of $X$ ($\forall$, $\exists$, or $L$), which is part of
$\text{Emb}_{X}$ but at different indices. We use notations
$\text{Msg}_{X \to Y}$ to denote messages from $X$ to $Y$. We also use notations
$\mathcal{M}_{X}$ to denote MLPs that generate messages from the embeddings of $X$, notations
$\mathcal{M}_{X \to Y}$ to denote MLPs that generate messages from the embeddings of $X$ for $Y$, notations
$\mathcal{L}_{X}$ to denote LSTMs that update embeddings of $X$ given incoming messages, and notations
$\mathcal{L}_{X \leftarrow Y}$ to denote LSTMs that update embeddings of $X$ given incoming messages from $Y$. We also use notations
$\mathbb{E}_{X}$ to denote adjacency matrix of $X$ ($\forall$, $\exists$, or $C$) and clauses, notations
$X \cdot Y$ to denote matrix multiplication of $X$ and $Y$, notations
$[X, Y]$ to denote matrix concatenation of $X$ and $Y$, and notations
$X^T$ to denote matrix transportation of $X$.

The simplest form of embedding of QBF (Model 1) is given below. 

$$\small
\ba{cl}
\textbf{Model 1:} \\ 
\text{Msg}_{\forall \to C} = \mathcal{M}_{\forall} (\text{Emb}_\forall) \\
\text{Msg}_{\exists \to C} = \mathcal{M}_{\exists} (\text{Emb}_\exists) \\
\text{Emb}_{C} = \mathcal{L}_{C} (\mathbb{E}_\forall \cdot \text{Msg}_{\forall \to C} +
                 \mathbb{E}_\exists \cdot \text{Msg}_{\exists \to C}) \\
\text{Msg}_{C \to L} = \mathcal{M}_{C} (\text{Emb}_{C}) \\
\text{Emb}_\forall = \mathcal{L}_\forall ([\mathbb{E}_\forall^T \cdot \text{Msg}_{C \to L}, \text{Emb}_{\neg \forall}]) \\
\text{Emb}_\exists = \mathcal{L}_\exists ([\mathbb{E}_\exists^T \cdot \text{Msg}_{C \to L}, \text{Emb}_{\neg \exists}]) \\
\ea
$$

In Model 2, we update the clause embedding by 2 LSTMs,
each of them take the messages from $\forall$ and $\exists$ literals separately.
% We switch the order of these 2 LSTMs in Model 3.

$$\small
\ba{cl}
\textbf{Model 2:} \\ 
\text{Msg}_{\forall \to C} = \mathcal{M}_{\forall} (\text{Emb}_\forall) \\
\text{Msg}_{\exists \to C} = \mathcal{M}_{\exists} (\text{Emb}_\exists) \\
\text{Emb}_{C} = \mathcal{L}_{C \leftarrow \forall} (\mathbb{E}_\forall \cdot \text{Msg}_{\forall \to C}) \\
\text{Emb}_{C} = \mathcal{L}_{C \leftarrow \exists} (\mathbb{E}_\exists \cdot \text{Msg}_{\exists \to C}) \\
\text{Msg}_{C \to L} = \mathcal{M}_{C} (\text{Emb}_{C}) \\
\text{Emb}_\forall = \mathcal{L}_\forall ([\mathbb{E}_\forall^T \cdot \text{Msg}_{C \to L}, \text{Emb}_{\neg \forall}]) \\
\text{Emb}_\exists = \mathcal{L}_\exists ([\mathbb{E}_\exists^T \cdot \text{Msg}_{C \to L}, \text{Emb}_{\neg \exists}]) \\
\ea
$$


% $$\small
% \ba{cl}
% \textbf{Model 2:} \\ 
% \text{Msg}_{\forall \to C} = \text{MLP}_\forall (\text{Emb}_\forall) \\
% \text{Message}_\exists = \text{MLP}_\exists (\text{Emb}_\exists) \\
% \text{Emb}_{c} = \text{LSTM}_{c\forall} (\text{EdgeMatrix}_\forall (\text{Message}_\forall)) \\
% \text{Emb}_{c} = \text{LSTM}_{c\exists} (\text{EdgeMatrix}_\exists (\text{Message}_\exists)) \\
% \text{Message}_{c} = \text{MLP}_{c} (\text{Emb}_{c}) \\
% \text{Emb}_\forall = \text{LSTM}_\forall ([\text{EdgeMatrix}_\forall^T (\text{Message}_{c}), \text{Emb}_{neg}]) \\
% \text{Emb}_\exists = \text{LSTM}_\exists ([\text{EdgeMatrix}_\exists^T (\text{Message}_{c}), \text{Emb}_{neg}]) \\
% \ea
% $$
% We can reverse the order of the two LSTM embedding updates.

We switch the order of these 2 LSTMs in Model 3.

$$\small
\ba{cl}
\textbf{Model 3:} \\ 
\text{Msg}_{\forall \to C} = \mathcal{M}_{\forall} (\text{Emb}_\forall) \\
\text{Msg}_{\exists \to C} = \mathcal{M}_{\exists} (\text{Emb}_\exists) \\
\text{Emb}_{C} = \mathcal{L}_{C \leftarrow \exists} (\mathbb{E}_\exists \cdot \text{Msg}_{\exists \to C}) \\
\text{Emb}_{C} = \mathcal{L}_{C \leftarrow \forall} (\mathbb{E}_\forall \cdot \text{Msg}_{\forall \to C}) \\
\text{Msg}_{C \to L} = \mathcal{M}_{C} (\text{Emb}_{C}) \\
\text{Emb}_\forall = \mathcal{L}_\forall ([\mathbb{E}_\forall^T \cdot \text{Msg}_{C \to L}, \text{Emb}_{\neg \forall}]) \\
\text{Emb}_\exists = \mathcal{L}_\exists ([\mathbb{E}_\exists^T \cdot \text{Msg}_{C \to L}, \text{Emb}_{\neg \exists}]) \\
\ea
$$

% $$\small
% \ba{cl}
% \textbf{Model 3:} \\ 
% \text{Message}_\forall = \text{MLP}_\forall (\text{Emb}_\forall) \\
% \text{Message}_\exists = \text{MLP}_\exists (\text{Emb}_\exists) \\
% \text{Emb}_{c} = \text{LSTM}_{c\exists} (\text{EdgeMatrix}_\exists (\text{Message}_\exists)) \\
% \text{Emb}_{c} = \text{LSTM}_{c\forall} (\text{EdgeMatrix}_\forall (\text{Message}_\forall)) \\
% \text{Message}_{c} = \text{MLP}_{c} (\text{Emb}_{c}) \\
% \text{Emb}_\forall = \text{LSTM}_\forall ([\text{EdgeMatrix}_\forall^T (\text{Message}_{c}), \text{Emb}_{neg}]) \\
% \text{Emb}_\exists = \text{LSTM}_\exists ([\text{EdgeMatrix}_\exists^T (\text{Message}_{c}), \text{Emb}_{neg}]) \\
% \ea
% $$
In Model 4 we concatenate the messages from $\forall$ and $\exists$ literals.

% Model 4 in main manuscript
$$\small
\ba{cl}
\textbf{Model 4:} \\ 
\text{Msg}_{\forall \to C} = \mathcal{M}_{\forall} (\text{Emb}_\forall) \\
\text{Msg}_{\exists \to C} = \mathcal{M}_{\exists} (\text{Emb}_\exists) \\
\text{Emb}_{C} = \mathcal{L}_{C} ([\mathbb{E}_\forall \cdot \text{Msg}_{\forall \to C},
                                   \mathbb{E}_\exists \cdot \text{Msg}_{\exists \to C}]) \\
\text{Msg}_{C \to L} = \mathcal{M}_{C} (\text{Emb}_{C}) \\
\text{Emb}_\forall = \mathcal{L}_\forall ([\mathbb{E}_\forall^T \cdot \text{Msg}_{C \to L}, \text{Emb}_{\neg \forall}]) \\
\text{Emb}_\exists = \mathcal{L}_\exists ([\mathbb{E}_\exists^T \cdot \text{Msg}_{C \to L}, \text{Emb}_{\neg \exists}]) \\
\ea
$$


% $$\small
% \ba{cl}
% \textbf{Model 4:} \\ 
% \text{Message}_\forall = \text{MLP}_\forall (\text{Emb}_\forall) \\
% \text{Message}_\exists = \text{MLP}_\exists (\text{Emb}_\exists) \\
% \text{Input}_c = [\text{EdgeMatrix}_\forall (\text{Message}_\forall),
%                   \text{EdgeMatrix}_\exists (\text{Message}_\exists)] \\
% \text{Emb}_{c} = \text{LSTM}_{c} (\text{Input}_c) \\
% \text{Message}_{c} = \text{MLP}_{c} (\text{Emb}_{c}) \\
% \text{Emb}_\forall = \text{LSTM}_\forall ([\text{EdgeMatrix}_\forall^T (\text{Message}_{c}), \text{Emb}_{neg}]) \\
% \text{Emb}_\exists = \text{LSTM}_\exists ([\text{EdgeMatrix}_\exists^T (\text{Message}_{c}), \text{Emb}_{neg}]) \\
% \ea
% $$

The performance of our GNN architectures improve greatly after we realize that
(in Model 5) we may also need to use different MLP modules to generate messages
from clauses to $\forall$ and $\exists$ literals. Note that this is also the model
we reported in the main paper, and the model we decided to use for all results reported
in main paper.


$$\small
\ba{cl}
\textbf{Model 5:} \\ 
\text{Msg}_{\forall\to C} = \mathcal{M}_\forall (\text{Emb}_\forall) \\
\text{Msg}_{\exists\to C} = \mathcal{M}_\exists (\text{Emb}_\exists) \\
\text{Emb}_{C} = \mathcal{L}_{C}([\mathbb{E}_\forall \cdot \text{Msg}_{\forall\to C},
                                  \mathbb{E}_\exists \cdot \text{Msg}_{\exists\to C}]) \\
\text{Msg}_{C\to\forall} = \mathcal{M}_{C\to\forall} (\text{Emb}_{C}) \\
\text{Msg}_{C\to\exists} = \mathcal{M}_{C\to\exists} (\text{Emb}_{C}) \\
\text{Emb}_\forall = \mathcal{L}_\forall ([\mathbb{E}_\forall^T
 \cdot \text{Msg}_{C\to\forall}, \text{Emb}_{\neg \forall}]) \\
\text{Emb}_\exists = \mathcal{L}_\exists ([\mathbb{E}_\exists^T
\cdot \text{Msg}_{C\to\exists}, \text{Emb}_{\neg \exists}]) \\
\ea
$$

We also explore the possibility (in Model 6) of having two embeddings for each clause, one
serving the $\forall$ literals and one serving the $\exists$ literals.
We need extra notations:
$\text{Emb}_{X \to Y}$ denotes embeddings of $X$ that serves $Y$.
$\mathcal{L}_{X \to Y}$ denotes LSTMs that updates embedding of $X$ that serves $Y$.

$$\small
\ba{cl}
\textbf{Model 6:} \\ 
\text{Msg}_{\forall\to C} = \mathcal{M}_\forall (\text{Emb}_\forall) \\
\text{Msg}_{\exists\to C} = \mathcal{M}_\exists (\text{Emb}_\exists) \\
\text{Emb}_{C \to \forall} = \mathcal{L}_{C \to \forall}([\mathbb{E}_\forall \cdot \text{Msg}_{\forall\to C},
                                                          \mathbb{E}_\exists \cdot \text{Msg}_{\exists\to C}]) \\
\text{Emb}_{C \to \exists} = \mathcal{L}_{C \to \exists}([\mathbb{E}_\forall \cdot \text{Msg}_{\forall\to C},
                                                          \mathbb{E}_\exists \cdot \text{Msg}_{\exists\to C}]) \\
\text{Msg}_{C\to\forall} = \mathcal{M}_{C\to\forall} (\text{Emb}_{C \to \forall}) \\
\text{Msg}_{C\to\exists} = \mathcal{M}_{C\to\exists} (\text{Emb}_{C \to \exists}) \\
\text{Emb}_\forall = \mathcal{L}_\forall ([\mathbb{E}_\forall^T
 \cdot \text{Msg}_{C\to\forall}, \text{Emb}_{\neg \forall}]) \\
\text{Emb}_\exists = \mathcal{L}_\exists ([\mathbb{E}_\exists^T
\cdot \text{Msg}_{C\to\exists}, \text{Emb}_{\neg \exists}]) \\
\ea
$$

% Model 6 in main manuscript
% $$\small
% \ba{cl}
% \textbf{Model 6:} \\
% \text{Message}_\forall = \text{MLP}_\forall (\text{Emb}_\forall) \\
% \text{Message}_\exists = \text{MLP}_\exists (\text{Emb}_\exists) \\
% \text{Input}_c = [\text{EdgeMatrix}_\forall (\text{Message}_\forall),
%                   \text{EdgeMatrix}_\exists (\text{Message}_\exists)] \\
% \text{Emb}_{c\forall} = \text{LSTM}_{c\forall} (\text{Input}_c) \\
% \text{Emb}_{c\exists} = \text{LSTM}_{c\exists} (\text{Input}_c) \\
% \text{Message}_{c\forall} = \text{MLP}_{c\forall} (\text{Emb}_{c\forall}) \\
% \text{Message}_{c\exists} = \text{MLP}_{c\exists} (\text{Emb}_{c\exists}) \\
% \text{Emb}_\forall = \text{LSTM}_\forall ([\text{EdgeMatrix}_\forall^T (\text{Message}_{c\forall}), \text{Emb}_{neg}]) \\
% \text{Emb}_\exists = \text{LSTM}_\exists ([\text{EdgeMatrix}_\exists^T (\text{Message}_{c\exists}), \text{Emb}_{neg}]) \\
% \ea
% $$

We further explore possibility (in Model 7) that our embedding scheme should
reflect a CEGAR cycle, which starts from $\forall$ variables (proposing
candidates), to clauses, to $\exists$ variables (finding counterexamples), back
to clauses, then back to $\forall$ variables. 
% In the early stage of our
% experiment, we gradually decide to focus on Model 5, as it is expressive enough
% to fit the training data, and simple enough for fast turn-out and minimal
% overfitting. Note that the mathmatical process of Model 2,3,4,6, and 7 are
% provided in supplementary manuscript instead.

$$\small
\ba{cl}
\textbf{Model 7:} \\ 
\text{Msg}_{\forall\to C} = \mathcal{M}_\forall (\text{Emb}_\forall) \\
\text{Emb}_{C \to \exists} = \mathcal{L}_{C \to \exists}(\mathbb{E}_\forall \cdot \text{Msg}_{\forall\to C}) \\
\text{Msg}_{C\to\exists} = \mathcal{M}_{C\to\exists} (\text{Emb}_{C \to \exists}) \\
\text{Emb}_\exists = \mathcal{L}_\exists ([\mathbb{E}_\exists^T
\cdot \text{Msg}_{C\to\exists}, \text{Emb}_{\neg \exists}]) \\
\\
\text{Msg}_{\exists\to C} = \mathcal{M}_\exists (\text{Emb}_\exists) \\
\text{Emb}_{C \to \forall} = \mathcal{L}_{C \to \forall}(\mathbb{E}_\exists \cdot \text{Msg}_{\exists\to C}) \\
\text{Msg}_{C\to\forall} = \mathcal{M}_{C\to\forall} (\text{Emb}_{C \to \forall}) \\
\text{Emb}_\forall = \mathcal{L}_\forall ([\mathbb{E}_\forall^T
 \cdot \text{Msg}_{C\to\forall}, \text{Emb}_{\neg \forall}]) \\
\ea
$$

% Model 7 in main manuscript
% $$\small
% \ba{cl}
% \textbf{Model 7:} \\
% \text{Message}_\forall = \text{MLP}_\forall (\text{Emb}_\forall) \\
% \text{Emb}_{c\exists} = \text{LSTM}_{c\exists} (\text{EdgeMatrix}_\forall (\text{Message}_\forall)) \\
% \text{Message}_{c\exists} = \text{MLP}_{c\exists} (\text{Emb}_{c\exists}) \\
% \text{Emb}_\exists = \text{LSTM}_\exists ([\text{EdgeMatrix}_\exists^T (\text{Message}_{c\exists}), \text{Emb}_{neg}]) \\
% \\
% \text{Message}_\exists = \text{MLP}_\exists (\text{Emb}_\exists) \\
% \text{Emb}_{c\forall} = \text{LSTM}_{c\forall} (\text{EdgeMatrix}_\exists (\text{Message}_\exists)) \\
% \text{Message}_{c\forall} = \text{MLP}_{c\forall} (\text{Emb}_{c\forall}) \\
% \text{Emb}_\forall = \text{LSTM}_\forall ([\text{EdgeMatrix}_\forall^T (\text{Message}_{c\forall}), \text{Emb}_{neg}]) \\
% \ea
% $$
% \\
% \clearpage

\section{Functions for Ranking Scores}

Function for candidate ranking scores based on hardness,
i.e. the number of models of reduced SAT formula.

\begin{python}
def n_model_2_ranking_score(n_models):
    if n_models <= 3: return 10.0 - n_models
    if n_models <= 5: return 6.0
    if n_models <= 8: return 5.0
    if n_models <= 12: return 4.0
    if n_models <= 16: return 3.0
    if n_models <= 21: return 2.0
    else: return 1.0
\end{python}

Function for candidate ranking scores in maxSAT-style,
i.e. based on the number of satisfied clauses.

\begin{python}
def n_clauses_2_ranking_score(n_clauses_list):
    n_clauses_min = min(n_clauses_list)
    return [max(1, 10 - n_clauses + n_clauses_min)
            for n_clauses in n_clauses_list]
\end{python}

Function for counterexample ranking scores based on unsatisfiability cores
and number of satisfied clauses.

\begin{python}
def unsat_core_2_ranking_score(core_index,
                               n_clauses_list):
    n_clauses_max = max(n_clauses_list)
    scores = [max(1, 8 - n_clauses_max + n_clauses)
              for n_clauses in n_clauses_list]
    scores = numpy.array(scores)
    scores[core_index] = 10
    return scores.tolist
\end{python}

Function for counterexample ranking scores in maxSAT-style,
i.e. based on the number of satisfied clauses.

\begin{python}
def n_clauses_2_ranking_score_counter(n_clauses_list):
    n_clauses_max = max(n_clauses_list)
    return [max(1, 10 - n_clauses_max + n_clauses)
            for n_clauses in n_clauses_list]
\end{python}


